Object Style Diffusion for Generalized Object Detection in Urban Scene

Object detection is a critical task in computer vision, with applications in various domains such as autonomous driving and urban scene monitoring. However, deep learning-based approaches often demand large volumes of annotated data, which are costly and difficult to acquire, particularly in complex and unpredictable real-world environments. This dependency significantly hampers the generalization capability of existing object detection techniques. To address this issue, we introduce a novel single-domain object detection generalization method, named GoDiff, which leverages a pre-trained model to enhance generalization in unseen domains. Central to our approach is the Pseudo Target Data Generation (PTDG) module, which employs a latent diffusion model to generate pseudo-target domain data that preserves source domain characteristics while introducing stylistic variations. By integrating this pseudo data with source domain data, we diversify the training dataset. Furthermore, we introduce a cross-style instance normalization technique to blend style features from different domains generated by the PTDG module, thereby increasing the detector's robustness. Experimental results demonstrate that our method not only enhances the generalization ability of existing detectors but also functions as a plug-and-play enhancement for other single-domain generalization methods, achieving state-of-the-art performance in autonomous driving scenarios.

==> tables/SingleDomain.tex <==
\begin{table}[t]
    \centering
        \caption{
Impact of Different Generation Domains on Model Performance (mAP).
    }
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{@{}c|ccccccccc@{}}
            % \toprule
            \shline
            \textbf{Generated Domain} & \makecell{Day\\Sunny}& \makecell{Night\\Sunny} & \makecell{Dusk\\Rainy} &\makecell{Night\\Rainy}   & \makecell{Day\\Foggy} \\
            \midrule
            /   &  50.2 &   31.8 & 26.0 & 12.1 & 32.0  \\
            Daytime-Sunny  & \underline{53.1} & 30.7 & 28.3 & 12.5 & 33.7 \\
            Daytime-Foggy  & 52.2 & 31.8 & 26.0 & 12.1 & \underline{35.0} \\
            Dusk-Rainy  & 53.7 & \underline{33.3} & \textbf{32.6} & 13.9 & 33.7 \\
            Night-Rainy  & 52.1 & 32.0 & 28.3 & 12.5 & 33.9 \\
            Night-Sunny  & 52.5 & 32.6 & 31.0 & \textbf{14.6} & 33.7 \\
            All  & \textbf{55.2} & \textbf{34.9} & \underline{31.7} & \underline{13.7} & \textbf{35.2} \\
            % \ding{52} & \ding{52} & \ding{52} & \underline{55.0} & \textbf{35.4} & \underline{32.1} & \textbf{15.0} & \textbf{35.9} \\
            % \bottomrule
            \shline
        \end{tabular}
    \end{adjustbox}

    \label{tab:ablation_study}
\end{table}

==> tables/class-wise.tex <==
% \begin{table*}[t] \centering
%     \caption{A two-column table.}
%     \label{tab:table8}
%     \resizebox{\textwidth}{!}{
%     \Huge
%         \begin{tabular}{c|*{7}{c}|*{7}{c}}
%         \toprule
%         & \multicolumn{7}{c}{Daytime-Foggy} 
%                                & \multicolumn{7}{c}{Night-Sunny}   \\
%                              Method  & Bus & Bike & Car & Motor & Person & Rider & Truck 
%                                & Bus & Bike & Car & Motor & Person & Rider & Truck \\
%         \midrule
%         S-DGOD    & 4.8 & -1.7 & -0.9 & 3.5 & -0.7 & 2.7 & 2.6 & 5.9 & 3.1 & -5.9 & 5.9 & -2.7 & 4.5 & 4.8  \\
%         % C-Gap     & 1.7 & 6.2 & 8.6 & 7.8 & 5.7 & 8.7 & -1.6 & -5.8 & 3.1   & 8.2 & 1.7 & 1.3 & -0.7 & -0.2   \\
%         SRCD     & 5.7 & 3.4 & 2.7 & 5.1 & 3.5 & 4.6 & 4.5 
%                  & 5.4 & 1.9 & 2.8 & 4.7 & 3.3 & 2.9 & 2.1  \\
%         % U-FRCNN     & 1.9 & 6.2 & 12.4 & 7.5 & 6.5 & 7.1 & 0.8 & 0.1 
%         %             & 6.9 & 16.3 & -2.8 & 12.8 & 7.2 & 4.4  \\
%         \midrule
%         GoDiff      & 1.9 & 0.1 & 5.9 & 0.4 & 1.5 & 1.8 & 2.8 & 1.1 
%                     & 8.3 & 2.0 & 3.9 & 5.1 & 3.6 & 4.3 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h] \centering
%     \caption{A two-column table.}
%     \label{tab:table8}
%     \resizebox{\textwidth}{!}{
%     \Huge
%         \begin{tabular}{c|*{7}{c}|*{7}{c}}
%         \toprule
%         & \multicolumn{7}{c}{Dusk-Rainy} 
%                                & \multicolumn{7}{c}{Night-Rainy}   \\
%                             Method   & Bus & Bike & Car & Motor & Person & Rider & Truck 
%                                & Bus & Bike & Car & Motor & Person & Rider & Truck \\
%         \midrule
%         S-DGOD    & 4.8 & -1.7 & -0.9 & 3.5 & -0.7 & 2.7 & 2.6 & 5.9 & 3.1 & -5.9 & 5.9 & -2.7 & 4.5 & 4.8  \\
%         % C-Gap     & 2.1 / 15.8 & 0.22 & 0.14 & 0.97 & 3.1 / 23.5 & 0.31 & 0.23 & 0.97 & 2.0 / 6.7   & 0.17 & 0.28 & 0.99 & 4.5 / 34.4 & 0.38  \\
%         SRCD     & 5.7 & 3.4 & 2.7 & 5.1 & 3.5 & 4.6 & 4.5 
%                  & 5.4 & 1.9 & 2.8 & 4.7 & 3.3 & 2.9 & 2.1  \\
%         % U-FRCNN     & 1.9 & 6.2 & 12.4 & 7.5 & 6.5 & 7.1 & 0.8 & 0.1 
%         %             & 6.9 & 16.3 & -2.8 & 12.8 & 7.2 & 4.4  \\
%         \midrule
%         GoDiff      & 9.8 & 6.1 & 6.6 & 2.7 & 6.7 & 3.6 & 7.8 & 6.9 
%                     & 1.9 & 6.1 & -0.3 & 0.2 & -0.1 & 4.3 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



\begin{table*}[ht] \centering
    \caption{Comparison of mAP gain variations across various categories on DWD datasets.}
    \label{tab:table8}
    \resizebox{\textwidth}{!}{
    \Huge
        \begin{tabular}{c|*{7}{c}|*{7}{c}|*{7}{c}|*{7}{c}}
        \shline
        & \multicolumn{7}{c}{Daytime-Foggy} 
                               & \multicolumn{7}{c}{Night-Sunny} & \multicolumn{7} {c}{Dusk-Rainy} & \multicolumn{7}{c}{Night-Rainy}  \\
                             Method  & Bus & Bike & Car & Motor & Person & Rider & Truck 
                               & Bus & Bike & Car & Motor & Person & Rider & Truck 
                               & Bus & Bike & Car & Motor & Person & Rider & Truck 
                               & Bus & Bike & Car & Motor & Person & Rider & Truck \\
        \midrule
        S-DGOD    & 4.8 & -1.7 & -0.9 & 3.5 & -0.7 & 2.7 & 2.6 & 5.9 & 3.1 & -5.9 & 5.9 & -2.7 & 4.5 & 4.8 & 4.8 & -1.7 & -0.9 & 3.5 & -0.7 & 2.7 & 2.6 & 5.9 & 3.1 & -5.9 & 5.9 & -2.7 & 4.5 & 4.8 \\
        % C-Gap     & 1.7 & 6.2 & 8.6 & 7.8 & 5.7 & 8.7 & -1.6 & -5.8 & 3.1   & 8.2 & 1.7 & 1.3 & -0.7 & -0.2   \\
        SRCD     & 5.7 & 3.4 & 2.7 & 5.1 & 3.5 & 4.6 & 4.5 
                 & 5.4 & 1.9 & 2.8 & 4.7 & 3.3 & 2.9 & 2.1& 5.7 & 3.4 & 2.7 & 5.1 & 3.5 & 4.6 & 4.5 
                 & 5.4 & 1.9 & 2.8 & 4.7 & 3.3 & 2.9 & 2.1  \\
        % U-FRCNN     & 1.9 & 6.2 & 12.4 & 7.5 & 6.5 & 7.1 & 0.8 & 0.1 
        %             & 6.9 & 16.3 & -2.8 & 12.8 & 7.2 & 4.4  \\
        \midrule
        GoDiff      & 1.9 & 0.1 & 5.9 & 0.4 & 1.5 & 1.8 & 2.8 & 1.1 
                    & 8.3 & 2.0 & 3.9 & 5.1 & 3.6 & 4.3& 9.8 & 6.1 & 6.6 & 2.7 & 6.7 & 3.6 & 7.8 & 6.9 
                    & 1.9 & 6.1 & -0.3 & 0.2 & -0.1 & 4.3 \\
        \shline
    \end{tabular}
    }
\end{table*}
